Aesthetic Text Logo Synthesis via Content-aware Layout Inferring

Text logo design heavily relies on the creativity and expertise of professional designers, in which arranging element layouts is one of the most important procedures. However, few attention has been paid to this task which needs to take many factors (e.g., fonts, linguistics, topics, etc.) into consideration. In this paper, we propose a content-aware layout generation network which takes glyph images and their corresponding text as input and synthesizes aesthetic layouts for them automatically. Specifically, we develop a dual-discriminator module, including a sequence discriminator and an image discriminator, to evaluate both the character placing trajectories and rendered shapes of synthesized text logos, respectively. Furthermore, we fuse the information of linguistics from texts and visual semantics from glyphs to guide layout prediction, which both play important roles in professional layout design. To train and evaluate our approach, we construct a dataset named as TextLogo3K, consisting of about 3,500 text logo images and their pixel-level annotations. Experimental studies on this dataset demonstrate the effectiveness of our approach for synthesizing visually-pleasing text logos and verify its superiority against the state of the art.

==> backup.tex <==
Logo design requires a lot of creativity from professional designers, where arranging element layouts is one of the most important procedures.
However, few attention has been paid to this task which needs to take many factors (e.g., fonts, semantics, topics, etc.) into consideration.
In this paper, we propose a novel layout generation network which takes glyph images as input and synthesizes aesthetic layouts for them automatically.\fixme{should not the input be pure text?}
The highlights of this paper are threefold. First, we propose a dual-discriminator module (i.e., image and sequence discriminator) to better evaluate the quality of synthesized layouts. Second, we propose an effective scheme for integrating both semantic and visual features of texts into the layouts. Third, we construct a text logo segmentation dataset, and make it public for benefiting the investigation of related research (e.g., text segmentation, font generation) in the community. \fixme{I suggest list these item in the end of introduction}
We conduct extensive experiments to demonstrate the effectiveness of our method.

\fixme{more approximately, we suggest writing it like this. In our approach, we develop a dual-discriminator module, including an image and a sequence discriminator. ...why we need two discriminators .... how does these two discriminators help to solve the problem. Furthermore, in professionally designed layouts, linguistics from texts and visual semantics play an important role. To mimic this kind of speciality, we xxxx (here gives what we do) and how does it work. To train and evaluate our approach, we construct a dataset, consisting of xxx (scale). Experimental studies on this dataset demonstrate the superiority of our approach. The code and dataset are released here.}\par

\fixme{we should place a teaser image (double column) here to impress the reviewers (if we could)}
